Learning Geometrically Consistent Mesh Corrections

Building good 3D maps is a challenging and expensive task, which requires high-quality sensors and careful, time-consuming scanning. We seek to reduce the cost of building good reconstructions by correcting views of existing low-quality ones in a post-hoc fashion using learnt priors over surfaces and appearance. We train a CNN model to predict the difference in inverse-depth from varying viewpoints of two meshes -- one of low quality that we wish to correct, and one of high-quality that we use as a reference. In contrast to previous work, we pay attention to the problem of excessive smoothing in corrected meshes. We address this with a suitable network architecture, and introduce a loss-weighting mechanism that emphasises edges in the prediction. Furthermore, smooth predictions result in geometrical inconsistencies. To deal with this issue, we present a loss function which penalises re-projection differences that are not due to occlusions. Our model reduces gross errors by 45.3%--77.5%, up to five times more than previous work.

==> sections/5_discussion.tex <==
\section{Discussion}


==> sections/old_related-work.tex <==
\section{Related Work}\label{sec:related-work}
This work is based on the mesh correction model proposed by \citeauthor{Tanner:2018:MeshedUp}{Tanner~\etal{}}.
As we operate on inverse-depth images to correct meshes, our work is similar to depth refinement.
Below, we review some of the literature on that topic, as well as some other methods that our system draws inspiration from.

\subsubsection*{Filtering and optimisation of depth}
Improving depth or disparity images is a well-researched area, with various methods proposed, some of which are guided by an additional aligned colour image.
The most straightforward unguided techniques are based on minimising either on a \ac{jbf} \citep{Tomasi:1998:JBF} when filtering, or \ac{tgv} \citep{Bredies:2010:TGV} for optimisation.
Guided techniques use another image aligned with the depth-map to inform the refinement.
The guide image is used especially around edges, to modulate the smoothing effect of filtering or optimisation.
For example, \cite{Kopf:2007:JBUpsample} or \cite{Matsuo:2013:WeightedJBF} propose variants of a \ac{jbf} for refining depth, while \cite{Tanner:2016:KeepGeometryInContext} demonstrates a \acs{tgv}-based method that uses both magnitude and direction of colour images to regularise depth maps.
An interesting combination of learning and optimisation is proposed by \cite{Riegler:2016:ATGVNet}.
The Primal-Dual algorithm \citep{Chambolle:2011:PrimalDual} normally employed for \ac{tgv} optimisation is unrolled and included into a \ac{cnn} model that learns to upsample depth images.
Our work is relies on an existing \threed{} reconstruction pipeline \citep{Tanner:2015:BORG}, in which some of these depth refinement techniques have already been employed.
We focus on post-processing meshes and fixing errors that cannot easily be fixed in single, live depth images.

\subsubsection*{Learnt depth refinement and completion}
Some methods for \emph{learning} depth map refinement and completion have been recently proposed.
\cite{Uhrig:2017:SparsityInvariant,Eldesokey:2018:UncertaintySparsity} propose \ac{cnn} model for solving the KITTI Depth Completion Challenge, where sparse depth maps produced from laser data are densified.
\cite{Hua:2018:NConvDepthCompletion} use normalised convolutions \citep{Knutsson:1993:NormalizedConv} to predict dense depth maps that have been sparsely sampled.
These methods all rely on having some sort of high-quality, usually laser, depth information (albeit sparse) at run-time, and are only designed to fill in the missing data.
In contrast, we only require high-quality data during training, and our method aims to refine depth from a low-quality mesh in a more general sense – both filling in blanks, as well as refining existing surfaces.

A few other methods more closely related in spirit to ours aim to learn depth refinement using meshes as reference.
\cite{Kwon:2015:DataDrivenDepth} use dictionary learning to model the statistical relationships between raw \textsc{rgb-d} images, and high-quality depth data obtained by fusing multiple depth maps with KinectFusion \citep{Newcombe:2011:KinectFusion}.
Two other recent works use fused \textsc{rgb-d} reconstruction to obtain high-quality reference data and train \ac{cnn}s to enhance depth.
\cite{Zhang:2018:DeepDepthCompletion} uses a colour image to predict normals and occlusion boundaries, supervised by the \threed{} reconstruction, and then formulates an optimisation problem to fill in holes in an aligned depth image.
\cite{Jeon:2018:ReconstructionPairwiseDataset} introduce a 4000-image dataset of raw/clean depth image pairs, and train a \ac{cnn} to enhance raw depth maps.
Furthermore, they show that \threed{} reconstructions can be obtained with fewer data and quicker when using their depth-enhancing network.
These methods all rely on live colour images to guide the refinement or completion of live depth.
That means that only limited data is available for training.
In contrast, our purely mesh-based formulation allows us to extract many more training pairs from any viewpoint, removing any viewpoint-specific bias that might otherwise surface while learning.

\subsubsection*{Learnt depth estimation}
Another related line of research has been monocular depth estimation, which inspires our choices of network architecture and the use of geometry as a source of self-supervision.
\cite{Godard:2017:UnsupervisedMonoDepth,Laina:2016:Deeper,Ummenhofer:2017:DeMoN,Zhou:2017:SfMLearner,Dharmasiri:2018:ENG,Mahjourian:2018:Vid2Depth,Klodt:2018:SfMFromSfM}, etc. propose various \ac{cnn} models for depth estimation from single colour images.
When explicit depth ground-truth is unavailable, the training is self-supervised using multiview geometry: the predicted depths and relative poses should maximise the photometric consistency of nearby input images.
In this work, we show how the photometric consistency loss can be adapted to ensure consistency between inverse-depth predictions directly, without need for colour images.

\subsubsection*{Learning introspection}
- a lot of the pixels are already correct: mask them and only correct the rest
- uncertaitny Kendall \cite{Kendall:2017:WhatUncertainties}
- robust loss Barron \cite{Barron:2017:AdaptiveRobustLoss}
- demo in practice \cite{Klodt:2018:SfMFromSfM}

As a simple way to offer our model some introspective capabilities, we predict a soft attention mask in addition to the error in inverse-depth.
This mask is used to modulate which parts of the error prediction are going to be applied.
\ssnotes{move this to method}
